Keep soft robots soft -- a data-driven based trade-off between feed-forward and feedback control

Tracking control for soft robots is challenging due to uncertainties in the system model and environment. Using high feedback gains to overcome this issue results in an increasing stiffness that clearly destroys the inherent safety property of soft robots. However, accurate models for feed-forward control are often difficult to obtain. In this article, we employ Gaussian Process regression to obtain a data-driven model that is used for the feed-forward compensation of unknown dynamics. The model fidelity is used to adapt the feed-forward and feedback part allowing low feedback gains in regions of high model confidence.

==> figure/var_gains.tex <==
\begin{tikzpicture}[auto, node distance=1.5cm,>=latex']
	\tikzstyle{block} = [draw, fill=white, rectangle,minimum height=2em, minimum width=6em]
	\tikzstyle{sum} = [draw, fill=white, circle, node distance=1cm]
	\tikzstyle{cross} = [draw, fill=black, circle,inner sep=1pt, node distance=1cm]
	\tikzstyle{input} = [coordinate]
	\tikzstyle{output} = [coordinate]
	\tikzstyle{mid} = [coordinate]

    % We start by placing the blocks
    \node [block, align=center] (ct) {$\scriptstyle \textsf{Estimated model}$};
    \node [block, below=1cm of ct.west, anchor=west, align=center] (model) {$\scriptstyle \textsf{GP model}$};
    \node [block, below of=model, node distance=1.3cm] (controller) {$\scriptstyle \textsf{Feedback}$};
    \node [coordinate, below right=0.2cm and -0.4cm of controller] (arrow) {};
    \node [sum, left of=controller,node distance=1.5cm,label={[label distance=0cm]240:-}] (sum) {};
    \node [input, name=input, left of=sum] {};
    \node [cross, left of=model, node distance=2cm] (cr) {};
    \node [sum, right of=model,node distance=2.5cm] (sum1) {};
	\node [block, right of=sum1,node distance=2cm] (system) {$\scriptstyle \textsf{Soft robot } \cref{for:dyn_model}$};
	\node [mid, below of=controller,node distance=0.8cm] (mid1) {};
	
	\draw [->] (cr) -- node {} (model);
	\draw [-] (input) -| node {} (cr);
    % Once the nodes are placed, connecting them is easy. 
    \draw [draw,->] (input) -- node {$\scriptstyle \y_d$} (sum);
    \draw [->] (sum) -- node {} (controller);
     \draw [->] (cr) |- node {} (ct);
    \draw [->] (controller) -| node {} (sum1);
    \draw [->] (model.south) -- node[ label={[xshift=-0.5cm, yshift=-0.3cm]$\scriptstyle \textsf{Variance }\,\Sigma$}] {} (controller.north) -- (arrow);
    \draw [->] (model) -- node {$\scriptstyle \textsf{Mean }\Mean$} (sum1);
    \draw [->] (ct) -| node {} (sum1);
    \draw [->] (sum1) -- node {$\scriptstyle \p$} (system);
     \draw [->] (system.south) |- node[pos=0.3,label=$\scriptstyle \y$]{} (mid1) -|(sum.south);
    %\draw [->] (system) -- node [name=y] {$y$}(output);
\end{tikzpicture}
